Status and prospects of the NEXT experiment for neutrinoless double beta decay searches

NEXT (Neutrino Experiment with a Xenon TPC) is an experimental program whose goals are to discover neutrinoless double beta decay using $^{136}$Xe in high pressure xenon TPCs with electroluminescent readout. In this paper, results from the NEXT-White detector, which is currently taking data at Laboratorio Subterr\'aneo de Canfranc (LSC) will be reported. The prospects for the NEXT-100 apparatus, scheduled to start operations in 2020, as well as the plans to extend the technology to large and ultra-low background detectors needed to fully explore the inverse hierarchy of neutrino masses, will also be briefly discussed.

==> NextLatexPackagesBase.tex <==
\usepackage{babel}
\usepackage[document]{ragged2e}

\usepackage{amsfonts}
\usepackage{wrapfig}
\usepackage{hyperref}

\usepackage{graphbox}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{amsmath,amssymb, gensymb}
\usepackage{natbib,hyperref}
\usepackage{url}
\usepackage{siunitx}
\sisetup{separate-uncertainty=true}
\usepackage{xspace}
\usepackage{microtype}
\usepackage{subfig}
\usepackage[useregional]{datetime2}
\usepackage{graphicx}
%\usepackage{subcaption}

